Inverse Scale Space Decomposition

We investigate the inverse scale space flow as a decomposition method for decomposing data into generalised singular vectors. We show that the inverse scale space flow, based on convex and absolutely one-homogeneous regularisation functionals, can decompose data represented by the application of a forward operator to a linear combination of generalised singular vectors into its individual singular vectors. We verify that for this decomposition to hold true, two additional conditions on the singular vectors are sufficient: orthogonality in the data space and inclusion of partial sums of the subgradients of the singular vectors in the subdifferential of the regularisation functional at zero. We also address the converse question of when the inverse scale space flow returns a generalised singular vector given that the initial data is arbitrary (and therefore not necessarily in the range of the forward operator). We prove that the inverse scale space flow is guaranteed to return a singular vector if the data satisfies a novel dual singular vector condition. We conclude the paper with numerical results that validate the theoretical results and that demonstrate the importance of the additional conditions required to guarantee the decomposition result.

==> numerics.tex <==
\section{Numerical Solution of the Inverse Scale Space Flow}
%In this section we want to discuss the numerical computation of solutions of the ISS flow (\ref{eq: ISSflow}), in order to verify our theoretical results. Subsequently we also want to discuss the numerical computation of singular vectors, and how the theoretical results of this paper may contribute to more sophisticated reconstruction methods.

%\subsection{Numerical Solution of the Inverse Scale Space Flow}
In order to verify the theoretical results provided in Section \ref{sec:decomp}, we need to be able to solve the ISS flow (\ref{eq: ISSflow}) numerically. In \cite{burger2013adaptive} it has been shown that solutions of (\ref{eq: ISSflow}) can be computed directly in case of $J(u) = \| u  \|_{\ell^1(\R^m)}$ via what has been termed the adaptive inverse scale space method (aISS). %The aISS method is given in Algorithm \ref{alg:aissalgorithm} for the sake of completeness. 
%\begin{algorithm}[H]
%	\caption{Adaptive Inverse Scale Space Method}		
%	\begin{algorithmic}
%		\State $1.$ \textbf{Parameters:} $K, \ f, \ \text{threshold} \geq 0$
%		\State $2.$ \textbf{Initialisation:} $t_1 = 1/\left\|K^T f\right\|_\infty, \ p(t_1) = t_1 ~K^T f, \ I_1 = \{ i \ | \ |p_i(t_1)| = 1 \}$
%			\While{$\| Ku(t_k) - f \|_2 > \text{threshold}$}
%				\vspace{0.1cm}
%				\State Compute $u(t_k) = \argmin_u \left\{ \|KP_{I_k}u - f\|_2^2 \right\}$ subject to $u(t_k) p(t_k) \geq 0$
%				\vspace{0.05cm}
%				\State Obtain $t_{k + 1} = \min\{ t ~|~t > t_k,  \exists j: |p_j(t)| = 1, u_j(t_k) = 0, p_j(t) \neq p_j(t_k) \}$
%				\vspace{0.05cm}
%				\State Update $p_j(t_{k + 1}) = p_j(t_k) + (t_{k+1}-t_k) e_j \cdot A^T (f - A u(t_k))$ for all $j$
%				\vspace{0.05cm}
%				\State Compute $I_{k + 1} = \{ i \ | \ |p_i(t_{k + 1})| = 1 \}$
%				\vspace{0.1cm}
%			\EndWhile
%			\State \Return $u(t_k)$
%	\end{algorithmic}
%	\label{alg:aissalgorithm}
%\end{algorithm}
%Here $P_{I_k}$ denotes the projection onto the index-set $I_k$. We are going to use Algorithm \ref{alg:aissalgorithm} in the following section in order to numerically support the necessity of the \eqref{eq: subdiff_cond}-condition as stated in Examples \ref{example: l1_convolution} and \ref{example: PartialSUB0Necessary}.\\
In \cite{moeller2013multiscale} the aISS has been extended to general polyhedral functionals $J$ and could therefore also be used to numerically verify the behaviour of functionals like the anisotropic total variation, for example. For arbitrary convex, absolutely one-homogeneous functionals $J$, however, there does not exist a way to efficiently compute the exact ISS solution at each time step numerically to the best of our knowledge. For simplicity we are going to restrict ourselves to the case of $J(u) = \| u \|_{\ell^1(\R^n)}$ for the numerical results.

%What is nevertheless possible due to Lemma \ref{lemma: FirstNonTrivialSol} is the numerical computation of the first non-trivial solution of the ISS flow. This may be sufficient to already verify if a violation of \eqref{eq: subdiff_cond} leads to a different ISS solution with respect to Theorem \ref{thm: ExactReconstruction}. In order to compute the first non-trivial ISS solution we could simply solve \eqref{eq: FirstISSsol}. However, we are going to choose a slightly easier way in order to avoid the computation of $\| K^* f \|_{\uc^*}$. Instead of computing a solution of \eqref{eq: FirstISSsol} we compute a solution of
%\begin{align}
%\tilde{u} \in \argmin_{u \in \ker(J)^{\perp}} \left\{ J(u) \quad \text{subject to} \quad \langle K^* f, u \rangle = c_0 \right\}. \label{eq:altFirstISSsol}
%\end{align}
%Here $c_0$ denotes the norm-inequality coefficient of \eqref{eq: NormIneqAssumption}. Problem \eqref{eq:altFirstISSsol} is a simple convex problem with a linear constraint, which can be solved efficiently by numerous standard solvers. We don't claim that $\tilde{u}$ and $u_1$ are the same, but we observe that their Bregman distance with respect to the subgradient $t_1 K^* f$ is zero:
%\begin{align*}
%0 \leq D_J^{t_1 K^* f}(\tilde{u}, u_1) &= J(\tilde{u}) - J(u_1) - t_1 \langle K^* f, \tilde{u} - u_1 \rangle\\
%&= \tilde{\mu} c_0 - t_1 \langle K^* f, u_1 \rangle - t_1 c_0 + t_1 \langle K^* f, u_1 \rangle\\
%&= t_1 ( \| K^* f \|_{\uc^*} \tilde{\mu} - c_0 ) \leq t_1 (c_0 - c_0 ) = 0 \, \text{,} 
%\end{align*}
%and hence we can conclude $D_J^{t_1 K^* f}(\tilde{u}, u_1) = 0$. Here we have made use of \mred{...} and the fact that $\tilde{\mu} K^*f \in \partial J(\tilde{u})$ implies $\tilde{\mu} \| K^* f \|_{\uc^*} \leq c_0$ by \textcolor{red}{(REF) to lemma - which is not proved yet}. \mred{Technically we still have to prove this.}

%\subsection{Bilevel Learning}
%To conclude this section we want to mention that there are also ways to address the problem of reverse engineering of regularisation methods for which given sets of functions are generalised singular vectors. A detailed analysis of this topic is beyond the scope of this paper, but we want to outline some basic bilevel optimisation strategies that could perform related tasks. \mbl{Short description \& bilevel references here!} \\
%
%Let $\{ g_i \}_{i = 1}^{m}$ be a set of functions and let $J(u; v) : \uc \times \mathcal{P} \rightarrow \R$ be a parametrised regularisation functional with parameters $v \in \mathcal{P}$ in some parameter space $\mathcal{P}$. 
%An example for such a regularisation functional could for instance be $J(u; v) = \| u \ast v \|_1$ as used in \mbl{Reference}, where $\ast$ denotes the convolution operator. Given such a set of functions and a parametrised regularisation functional, we can try to optimise the parameters according to the following bilevel optimisation strategy:
%\begin{align}
%\hat{v} &\in \argmin_{v \in \mathcal{P}} \left\{ \frac{1}{2} \sum_{i = 1}^m \| R_i(v) - g_i \|_{L^2(\Omega)}^2 + G(v) \right\}
%\intertext{subject to}
%R_i(v) &= \argmin_{u \in \dom(J)} \left\{ \frac{\gamma}{2} \| u - g_i \|_{L^2(\Omega)}^2 - \frac{J(g_i; v)}{\| Kg_i \|_{\hc}^2} \langle u, K^* Kg_i \rangle + J(u; v) \right\}
%\end{align}
%for all $i \in \{1; n\}$. Here $G:\mathcal{P} \rightarrow \R \cup \{ + \infty \}$ denotes a generic regularisation functional guaranteeing a certain regularity of the optimal parameters $\hat{v}$ and $\gamma > 0$ is a parameter chosen in advance. \\
%
%Given enough degrees of freedom for the parameters $v\in\mathcal{P}$, the optimal parameters $\hat{v}$ are ideally chosen such that $R_i(\hat{v}) = g_i$ for all $i \in \{1; n\}$, and hence, the $g_i$'s then represent generalised singular vectors with respect to the functional $J(u; \hat{v})$, i.e. $\lambda_i K^* K g_i \in \partial J(g_i; \hat{v})$ and $\lambda_i = J(g_i; \hat{v})/\| Kg_i\|_{\hc}^2$. \\
%
%Given that potential singular vectors are probably not easily at hand, using a strategy that exploits the scale-space nature may be more applicable. Based on the findings in the previous sections, it seems sensible to look into bilevel frameworks of the form
%\begin{align*}
%\hat{v} &\in \argmin_{v \in \mathcal{P}} \left\{ \frac{1}{2} \sum_{i = 1}^m \| R_i(v) - g_i \|_{L^2(\Omega)}^2 + G(v) \right\}
%\end{align*}
%\mbl{Martin to continue here!}
